Communication-optimal parallel and sequential QR and LU factorizations: theory and practice

We present parallel and sequential dense QR factorization algorithms that are both optimal (up to polylogarithmic factors) in the amount of communication they perform, and just as stable as Householder QR. Our first algorithm, Tall Skinny QR (TSQR), factors m-by-n matrices in a one-dimensional (1-D) block cyclic row layout, and is optimized for m >> n. Our second algorithm, CAQR (Communication-Avoiding QR), factors general rectangular matrices distributed in a two-dimensional block cyclic layout. It invokes TSQR for each block column factorization.

==> Tables/seq-caqr.tex <==
\begin{table}[h]
\small
\centering
\begin{tabular}{l | l}
            & Sequential CAQR \\ \hline
\# messages & $\frac{3}{2} P (P_c - 1)$ \\ 
\# words    & $\frac{3}{2} mn \left( P_c + \frac{4}{3} \right)
               - \frac{n^2 P_c}{2} + O\left( n^2 + n P \right)$ \\ 
\# flops    & $2mn^2 - \frac{2}{3} n^3$ \\ \hline \hline
             & \texttt{PFDGEQRF} \\ \hline
\# messages & $\frac{n}{2bc} + 2\frac{n}{c} - \frac{n}{2b}$ \\
\# words    & $\left( 
                   \frac{3mn}{2} - \frac{3n^2}{4}
               \right)
               + \frac{bn}{4}
               - \frac{13 cn}{12}
               + \frac{1}{c} \left(
                   \frac{mn^2}{2} 
                   - \frac{n^3}{6}
                   + \frac{n^2}{2} 
                   - \frac{bn^2}{4}
               \right)$ \\
\# flops    & $2mn^2 - \frac{2}{3} n^3$ \\ 
\end{tabular}
\caption{Performance models of sequential
  CAQR and the sequential out-of-DRAM QR factorization
  \lstinline!PFDGEQRF!, when factoring an $m \times n$ matrix.  In the
  case of sequential CAQR, the matrix is arranged in a 2-D block
  cyclic layout on a $P_r \times P_c$ grid with $m/P_r \times n/P_c$ 
  blocks.  We assume $m \geq n$ and $m/P_r
  \geq n/P_c$.  In the case of \lstinline!PFDGEQRF!, $b$ is the width
  of the left panel and $c$ is the width of the current panel being
  factored (the algorithm is left-looking).  In this table only, 
  ``flops'' includes floating-point divisions as well as additions 
  and multiplications.  Some lower-order terms are omitted.}
\label{tbl:CAQR:seq:model}
\end{table}

\endinput


==> Tables/summary-caqr.tex <==
\begin{table}[h]
\small
\centering
\begin{tabular}{l | l l}
\multicolumn{3}{c}{Parallel} \\ 
     & CAQR & ScaLAPACK \\ \hline
\# messages & $\frac{3}{8} \sqrt{P} \log^3 P$   
            & $\frac{5n}{4} \log^2 P$ \\       % fixed 11 Jul 2008
\# words & $\frac{3n^2}{4 \sqrt{P}} \log P$    % fixed 11 Jul 2008
         & $\frac{3n^2}{4 \sqrt{P}} \log P$ \\
\# flops & $\frac{4n^3}{3P}$    
         & $\frac{4n^3}{3P}$ \\ \hline \hline
\multicolumn{3}{c}{Sequential} \\
     & CAQR & ScaLAPACK \\ \hline
\# messages & $12 \frac{n^3}{W^{3/2}}$
            & $\frac{n^3}{2W}$ \\ 
\# words & $3 \frac{n^3}{\sqrt{W}}$ 
         & $\frac{n^4}{3W} + \frac{3n^2}{4}$ \\
\# flops & $\frac{4}{3} n^3$    
         & $\frac{4}{3} n^3$ \\ 
\end{tabular}
  \caption{Performance models of CAQR on a square $n \times n$
    matrix.  In the parallel case, the optimal $2-D$ block cyclic
    layout on $P$ processors is chosen, and in the sequential case,
    the optimal layout for a fast memory size of $W$ floating-point
    words is chosen.  In the parallel case, everything (messages, 
    words, and flops) is counted along the critical path.  Block
    dimensions for the sequential algorithm are $n/\sqrt{P}$ by 
    $n/\sqrt{P}$, and for the parallel algorithm are given in Table
    \ref{tbl:CAQR:par:model:opt}.  For the performance model when
    using square blocks of any dimension, refer to Equation
    \eqref{Eq:ap_time_latavoidQR} in Appendix \ref{S:CAQR-par-detailed}.}
\label{tbl:CAQR:perfmodel-summary}
\end{table}

\endinput


==> Tables/summary-tsqr.tex <==
\begin{table}[h]
\small
\centering
\begin{tabular}{l | l l}
 \multicolumn{3}{c}{Parallel} \\
 & TSQR & ScaLAPACK \\ \hline
\# messages & $\log P$ 
            & $2n \log P$ \\
\# words & $\frac{n^2}{2} \log P$ 
         & $\frac{n^2}{2} \log P$ \\
\# flops & $\frac{2mn^2}{P} + \frac{2}{3}n^3 \log P$ 
         & $\frac{2mn^2}{P} + \frac{n^2}{2}\log P$  \\ \hline \hline
 \multicolumn{3}{c}{Sequential} \\
 & TSQR & ScaLAPACK \\ \hline 
\# messages & $\frac{2mn}{W - \frac{n(n+1)}{2}}$
            & $\frac{2mn}{W} + \frac{mn^2}{2W}$ \\ 
\# words & $2mn 
            + \frac{mn^2}{\widetilde{W}}
            - \frac{n(n+1)}{2}$
         & $\frac{m^2 n^2}{2W} 
            - \frac{m n^3}{6 W}
            + \frac{3mn}{2}
            - \frac{3n^2}{4}$ \\
\# flops & $2mn^2 - \frac{2n^3}{3}$
         & $2mn^2 - \frac{2n^3}{3}$  \\
\end{tabular}
\caption{Performance models of the TSQR and ScaLAPACK QR
  factorizations on an $m \times n$ matrix with $P$ processors (in the
  parallel case) or a fast memory size of $W$ floating-point words (in 
  the sequential case), with $\tildetilde{W} = W - n(n+1)/2$.  Units
  of message volume are number of floating-point words transferred.  
  In the parallel case, everything (messages, words, and flops) is 
  counted along the critical path.  We assume $m \gg n$.}
\label{tbl:TSQR:perfmodel-summary}
\end{table}

\endinput

